LLaMA Pro: Progressive LLaMA with Block Expansion

Humans generally acquire new skills without compromising the old; however, the opposite holds for Large Language Models (LLMs), e.g., from LLaMA to CodeLLaMA. To this end, we propose a new post-pretraining method for LLMs with an expansion of Transformer blocks. We tune the expanded blocks using only new corpus, efficiently and effectively improving the model's knowledge without catastrophic forgetting. In this paper, we experiment on the corpus of code and math, yielding LLaMA Pro-8.3B, a versatile foundation model initialized from LLaMA2-7B, excelling in general tasks, programming, and mathematics. LLaMA Pro and its instruction-following counterpart (LLaMA Pro-Instruct) achieve advanced performance among various benchmarks, demonstrating superiority over existing open models in the LLaMA family and the immense potential of reasoning and addressing diverse tasks as an intelligent agent. Our findings provide valuable insights into integrating natural and programming languages, laying a solid foundation for developing advanced language agents that operate effectively in various environments.

==> table/trace.tex <==

\begin{table}[t]
\centering

\begin{tabular}{c|cc}
\toprule
\textbf{Method} & \textbf{Overall Performance (OP)}  & \textbf{Backward Transfer (BWT)}\\
\midrule
LoRA & 37.1 & -17.3\% \\
SeqFT & 45.5 & -14.7\% \\
Block Expansion & \textbf{46.5} & \textbf{-14.3\%} \\
% \instruct & 6.32 \\
% LLaMA2-7B-Chat & 6.27 \\
% Vicuna-7B & 6.17 \\
% CodeLLaMA-7B-Instruct & 5.71 \\
% Alpaca-13B & 4.53 \\
% \midrule
\bottomrule
\end{tabular}
\caption{Performance comparison of various training strategies on the TRACE benchmark following their continual learning phase with LLaMA2-7B. The table presents the Overall Performance (OP) and Backward Transfer (BWT) scores for each strategy, demonstrating the superior adaptability of the proposed block expansion training approach. }
\label{tab:trace}
% \vspace{-3mm}
\end{table}

==> table/trace_data.tex <==
\begin{table}[t]
\centering
\begin{tabular}{@{}llllll@{}}
\toprule
Dataset                         & Source       & Avg len & Metric          & Language & \#data \\ \midrule
\textit{Domain-specific}        &              &         &                 &          &        \\
ScienceQA                       & Science      & 210     & Accuracy        & English  & 5,000  \\
FOMC                            & Finance      & 51      & Accuracy        & English  & 5,000  \\
MeetingBank                     & Meeting      & 2853    & ROUGE-L         & English  & 5,000  \\ \midrule
\textit{Multi-lingual}          &              &         &                 &          &        \\
C-STANCE                        & Social media & 127     & Accuracy        & Chinese  & 5,000  \\
20Minuten                       & News         & 382     & SARI            & Germany  & 5,000  \\ \midrule
\textit{Code completion}        &              &         &                 &          &        \\
Py150                           & Github       & 422     & Edim similarity & Python   & 5,000  \\ \midrule
\textit{Mathematical reasoning} &              &         &                 &          &        \\
NumGLUE-cm                      & Math         & 32      & Accuracy        & English  & 5,000  \\
NumGLUE-ds                      & Math         & 21      & Accuracy        & English  & 5,000  \\ \bottomrule
\end{tabular}
\caption{An overview of dataset statistics in TRACE. 'Source' indicates the context's origin. 'Avg len' represents word count for English, German, and code datasets, and character count for Chinese. 'SARI' is a score specific to simplification.}
\label{tab:trace_data}
\end{table}

==> table/trace_detail.tex <==
\begin{table}[h]
\centering
\resizebox{0.7\linewidth}{!}
{
\begin{tabular}{@{}lllllllll@{}}
\toprule
Task\textbackslash{}Round & 1     & 2     & 3     & 4     & 5                           & 6     & 7     & 8     \\ \midrule
C-STANCE                  & 0.5 & 0.27 & 0.28  & 0.31 & 0.01 & 0.51 & 0.44  & 0.27   \\
FOMC                      & -     & 0.69 & 0.61 & 0.57 & 0.0 & 0.44 & 0.51  & 0.46 \\
MeetingBank               & -     & -     & 0.472 & 0.287  & 0.159 & 0.111 & 0.14 & 0.139 \\
Py150                     & -     & -     & -     & 0.61 & 0.294 & 0.551 & 0.547 & 0.364 \\
ScienceQA                 & -     & -     & -     & -     & 0.68 & 0.6 & 0.59 & 0.54  \\
NumGLUE-cm                & -     & -     & -     & -     & - & 0.395 & 0.309 & 0.272 \\
NumGLUE-ds                & -     & -     & -     & -     & - & -     & 0.59 & 0.51 \\
20Minuten                 & -     & -     & -     & -     & - & -     & -     & 0.414 \\ \midrule
OP                   &       &       &       &       &                             &       &       & 0.371 \\
BWT                       &       &       &       &       &                             &       &       & -0.173   \\ \bottomrule
\end{tabular}
}
\caption{Detailed results of sequentially LoRA training of LLaMA2-7B.}

\end{table}

\begin{table}[h]

\centering
\resizebox{0.7\linewidth}{!}
{
\begin{tabular}{@{}lllllllll@{}}
\toprule
Task\textbackslash{}Round & 1     & 2     & 3     & 4     & 5                           & 6     & 7     & 8     \\ \midrule
C-STANCE                  & 0.6 & 0.43 & 0.49  & 0.49 & 0.5 & 0.49 & 0.48  & 0.53   \\
FOMC                      & -     & 0.8 & 0.46 & 0.47 & 0.0 & 0.47 & 0.5  & 0.51 \\
MeetingBank               & -     & -     & 0.523 & 0.338  & 0.344 & 0.392 & 0.396 & 0.371 \\
Py150                     & -     & -     & -     & 0.594 & 0.265 & 0.561 & 0.566 & 0.575 \\
ScienceQA                 & -     & -     & -     & -     & 0.87 & 0.83 & 0.58 & 0.55  \\
NumGLUE-cm                & -     & -     & -     & -     & - & 0.383 & 0.198 & 0.210 \\
NumGLUE-ds                & -     & -     & -     & -     & - & -     & 0.64 & 0.49 \\
20Minuten                 & -     & -     & -     & -     & - & -     & -     & 0.407 \\ \midrule
OP                   &       &       &       &       &                             &       &       & 0.455 \\
BWT                       &       &       &       &       &                             &       &       & -0.147   \\ \bottomrule
\end{tabular}
}
\caption{Detailed results of sequentially fine-tuning of LLaMA2-7B.}

\end{table}

\begin{table}[h]

\centering
\resizebox{0.7\linewidth}{!}
{
\begin{tabular}{@{}lllllllll@{}}
\toprule
Task\textbackslash{}Round & 1     & 2     & 3     & 4     & 5                           & 6     & 7     & 8     \\ \midrule
C-STANCE                  & 0.65 & 0.52 & 0.52  & 0.52 & 0.28 & 0.52 & 0.5  & 0.57   \\
FOMC                      & -     & 0.8 & 0.49 & 0.45 & 0.0 & 0.44 & 0.46  & 0.45 \\
MeetingBank               & -     & -     & 0.512 & 0.363  & 0.338 & 0.383 & 0.393 & 0.38 \\
Py150                     & -     & -     & -     & 0.593 & 0.366 & 0.531 & 0.53 & 0.548 \\
ScienceQA                 & -     & -     & -     & -     & 0.89 & 0.8 & 0.6 & 0.63  \\
NumGLUE-cm                & -     & -     & -     & -     & - & 0.333 & 0.185 & 0.198 \\
NumGLUE-ds                & -     & -     & -     & -     & - & -     & 0.68 & 0.54 \\
20Minuten                 & -     & -     & -     & -     & - & -     & -     & 0.408 \\ \midrule
OP                   &       &       &       &       &                             &       &       & 0.465 \\
BWT                       &       &       &       &       &                             &       &       & -0.143   \\ \bottomrule
\end{tabular}
}
\caption{Detailed results of sequentially block expansion training of LLaMA2-7B.}

\end{table}

